BiNet: Degraded-Manuscript Binarization in Diverse Document Textures and Layouts using Deep Encoder-Decoder Networks

Handwritten document-image binarization is a semantic segmentation process to differentiate ink pixels from background pixels. It is one of the essential steps towards character recognition, writer identification, and script-style evolution analysis. The binarization task itself is challenging due to the vast diversity of writing styles, inks, and paper materials. It is even more difficult for historical manuscripts due to the aging and degradation of the documents over time. One of such manuscripts is the Dead Sea Scrolls (DSS) image collection, which poses extreme challenges for the existing binarization techniques. This article proposes a new binarization technique for the DSS images using the deep encoder-decoder networks. Although the artificial neural network proposed here is primarily designed to binarize the DSS images, it can be trained on different manuscript collections as well. Additionally, the use of transfer learning makes the network already utilizable for a wide range of handwritten documents, making it a unique multi-purpose tool for binarization. Qualitative results and several quantitative comparisons using both historical manuscripts and datasets from handwritten document image binarization competition (H-DIBCO and DIBCO) exhibit the robustness and the effectiveness of the system. The best performing network architecture proposed here is a variant of the U-Net encoder-decoders.

==> tex/results-old-delete.tex <==
\section{OLD Results DELETE later}
The results were evaluated on several test images. We compare the results of the proposed method to the following traditional methods:
\begin{itemize}
	\item Otsu
	\item Local Otsu
	\item Sauvola
	\item Niblack
\end{itemize}



\begin{figure}[]
	\centering
	
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/example/1082_1_color.jpg}}
		\caption{Color image of plate P1082}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/example/1082_1_fused.jpg}}
		\caption{Fused image of plate P1082}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}	
		\fbox{\includegraphics[width=.98\linewidth]{images/example/1082_1_result.jpg}}
		\caption{Binarized image using our method}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}	
		\fbox{\includegraphics[width=.98\linewidth]{images/example/label.png}}
		\caption{Ground-truth}	
	\end{subfigure}
	\caption{Test results of our trained model.}
	\label{fig:results}
\end{figure}


\subsection{Comparision with traditional methods}
We compared our method to traditional binarization methods, namely Otsu, local Otsu, Niblack and Sauvola. Figure \ref{fig:comp_trad} shows this comparison on the full image. Figure \ref{fig:comp_trad_zoom} shows this comparison on a crop from the centre of this image.

\begin{figure}[]
	\centering
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/comparison_traditional/otsu.png} }
		\subcaption{Otsu}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/comparison_traditional/local_otsu.png} }
		\subcaption{Local Otsu}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/comparison_traditional/niblack.png} }
		\subcaption{Niblack}	
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}	
		\fbox{\includegraphics[width=.98\linewidth]{images/comparison_traditional/sauvola.png} }
		\subcaption{Sauvola}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}	
		\fbox{\includegraphics[width=.98\linewidth]{images/comparison_traditional/result.jpg} }
		\subcaption{Our method}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}	
		\fbox{\includegraphics[width=.98\linewidth]{images/comparison_traditional/label.png} }
		\subcaption{Target}
	\end{subfigure}
	\caption{Comparison of our method with traditional methods for image plate P1082.}
	\label{fig:comp_trad}
\end{figure}

\begin{figure}[]
	\centering
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[trim=1400 1200 1600 1000,clip,width=.98\linewidth]{images/comparison_traditional/otsu.png} }
		\subcaption{Otsu}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[trim=1400 1200 1600 1000,clip,width=.98\linewidth]{images/comparison_traditional/local_otsu.png} }
		\subcaption{Local Otsu}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[trim=1400 1200 1600 1000,clip,width=.98\linewidth]{images/comparison_traditional/niblack.png} }
		\subcaption{Niblack}	
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}	
		\fbox{\includegraphics[trim=1400 1200 1600 1000,clip,width=.98\linewidth]{images/comparison_traditional/sauvola.png} }
		\subcaption{Sauvola}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}	
		\fbox{\includegraphics[trim=1400 1200 1600 1000,clip,width=.98\linewidth]{images/comparison_traditional/result.jpg} }
		\subcaption{Our method}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}	
		\fbox{\includegraphics[trim=1400 1200 1600 1000,clip,width=.98\linewidth]{images/comparison_traditional/label.png} }
		\subcaption{Target}
	\end{subfigure}
	\caption{Comparison of our method with traditional methods on a zoomed part of the image plate P1082.}
	\label{fig:comp_trad_zoom}
\end{figure}

\subsection{Comparison of gray/fused/color}
We trained models on grayscale images, color images and fused images. Figure \ref{fig:gcf_comp} shows the full images compared, while figure \ref{fig:gcf_comp_zoom} shows a crop from a part of the image.

\begin{figure}[]
	\centering
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/comparison_image_types/grayscale.png} }
		\subcaption{Grayscale}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/comparison_image_types/color.png} }
		\subcaption{Color}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/comparison_image_types/fused.png} }
		\subcaption{Fused}	
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}	
		\fbox{\includegraphics[width=.98\linewidth]{images/comparison_image_types/label.png} }
		\subcaption{Target}
	\end{subfigure}
	\caption{Comparison of test results from models trained on grayscale, colour and fused train images}
	\label{fig:gcf_comp}
\end{figure}

\begin{figure}[]
	\centering
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[trim=1800 1800 1100 250,clip,width=.98\linewidth]{images/comparison_image_types/grayscale.png} }
		\subcaption{Grayscale}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[trim=1800 1800 1100 250,clip,width=.98\linewidth]{images/comparison_image_types/color.png} }
		\subcaption{Color}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[trim=1800 1800 1100 250,clip,width=.98\linewidth]{images/comparison_image_types/fused.png} }
		\subcaption{Fused}	
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}	
		\fbox{\includegraphics[trim=1800 1800 1100 250,clip,width=.98\linewidth]{images/comparison_image_types/label.png} }
		\subcaption{Target}
	\end{subfigure}
	\caption{Comparison of test results from models trained on grayscale, colour and fused train images on a cropped part of the image}
	\label{fig:gcf_comp_zoom}
\end{figure}

\subsection{Comparison of original model with our model}

\begin{figure}[]
	\centering
	\begin{subfigure}{.14\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/comparison_models/original.png} }
		\subcaption{cGAN model}
	\end{subfigure}
	\begin{subfigure}{.14\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/comparison_models/l1.png} }
		\subcaption{Proposed model}
	\end{subfigure}
	\begin{subfigure}{.14\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/comparison_models/label.png} }
		\subcaption{Target}	
	\end{subfigure}
	\caption{Comparison between models}
	\label{fig:model_comp}
\end{figure}

\begin{figure}[]
	\centering
	\begin{subfigure}{.14\textwidth}
		\fbox{\includegraphics[trim=1400 1200 1600 1000,clip,width=.98\linewidth]{images/comparison_models/original.png} }
		\subcaption{cGAN model}
	\end{subfigure}
	\begin{subfigure}{.14\textwidth}
		\fbox{\includegraphics[trim=1400 1200 1600 1000,clip,width=.98\linewidth]{images/comparison_models/l1.png} }
		\subcaption{Proposed model}
	\end{subfigure}
	\begin{subfigure}{.14\textwidth}
		\fbox{\includegraphics[trim=1400 1200 1600 1000,clip,width=.98\linewidth]{images/comparison_models/label.png} }
		\subcaption{Target}	
	\end{subfigure}
	\caption{Comparison between models, crop from centre}
	\label{fig:model_comp_zoom}
\end{figure}
\subsection{Monkgrid image}

\begin{figure}[]
	\centering
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[trim=0 0 1200 0,clip,width=.98\linewidth]{images/monkgrid/monkgrid.png} }
		\subcaption{Input}
	\end{subfigure}
	\begin{subfigure}{.22\textwidth}
		\fbox{\includegraphics[trim=0 0 1200 0,clip,width=.98\linewidth]{images/monkgrid/output.png} } 
		\subcaption{Model output}
	\end{subfigure}
	\caption{Result of our model trained on Monk images for various documents}
	\label{fig:monkgrid}
\end{figure}

\subsection{DIBCO}
We trained our model on the DIBCO datasets from 2009 to 2014 and then tested it on the DIBCO datasets from 2016 and 2017. Figure \ref{fig:dibco1} shows the first image from the 2016 dataset and figure \ref{fig:dibco2} shows the first image from the 2017 dataset.

\begin{figure}[]
	\centering
	\begin{subfigure}{.14\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/dibco/dibco1.png} }
		\subcaption{Input}
	\end{subfigure}
	\begin{subfigure}{.14\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/dibco/output1.jpg} }
		\subcaption{Result}	
	\end{subfigure}
	\begin{subfigure}{.14\textwidth}	
		\fbox{\includegraphics[width=.98\linewidth]{images/dibco/gt1.png} }
		\subcaption{Ground truth}
	\end{subfigure}
	\caption{DIBCO 2016 image 1}
	\label{fig:dibco1}
\end{figure}

\begin{figure}[h]
	\centering
	\begin{subfigure}{.14\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/dibco/dibco2.png} }
		\subcaption{Input}
	\end{subfigure}
	\begin{subfigure}{.14\textwidth}
		\fbox{\includegraphics[width=.98\linewidth]{images/dibco/output2.jpg} }
		\subcaption{Result}	
	\end{subfigure}
	\begin{subfigure}{.14\textwidth}	
		\fbox{\includegraphics[width=.98\linewidth]{images/dibco/gt2.png} }
		\subcaption{Ground truth}
	\end{subfigure}
	\caption{DIBCO 2017 image 1}
	\label{fig:dibco2}
\end{figure}

\subsection{DIBCO measures}
Four measures were compared for DIBCO 2017:
F-measure, pseudo-Fmeasure, PSNR, DRD. The
F-measure measure, is calculated from a formula
false and true negatives and positives. The pseudo Fmeasure is calculated similarly to the F-measure
but has an additional weight term. This weight is
based on the distance from the edge of the nearest
painted shape. the PSNR or peak signal to noise ratio, the simplest explanation is that it determines
the similarity between the images. Lastly the DRD
or distance reciprocal distortion is measures the distortion, which correlates with human visual perception (Pratikakis et al., 2017).

For local Otsu, Sauvola and Niblack, a window size of 255x255 was used. We evaluated these with the following measures used in the H-DIBCO contest for handwritten document image binarization \cite{dibco2016}:
\begin{itemize}
	\item F-measure
	\item Pseudo F-measure
	\item Peak signal-to-noise ratio (PSNR)
	%\item Negative rate metric (NRM) not in dibco 2016
	%\item Misclassification penalty metric (MPM) not in dibco 2016
	\item Distance Reciprocal Distortion Metric (DRD)
\end{itemize}

Table \ref{tab:results} shows the results, where each value is the average of the 11 images. 

\begin{table}[h]
	\caption{Results of the methods, old DELETE}
	\label{tab:results}
	\begin{tabular}{l|lllll}
		& Otsu    & Local Otsu & Sauvola & Niblack & \textbf{Proposed} \\ \hline
		F-measure  & 0.07265 & 0.51266    & 0.19074 & 0.15676 & \textbf{0.65765}  \\
		pF-measure & 0.27118 & 0.52280    & 0.24581 & 0.14138 & \textbf{0.65535}  \\
		PSNR       & 1.55566 & 14.78624   & 6.27023 & 4.90463 & \textbf{17.54508} \\
		%NRM        & 0.50156 & 0.24226    & 0.44956 & 0.46181 & \textbf{0.02739}  \\
		%MPM        & 0.44865 & 0.00064    & 0.07627 & 0.19015 & \textbf{0.00012}  \\
		DRD        & 0.00010 & 0.01080    & 0.00001 & 0.00001 & \textbf{0.06507} 
	\end{tabular}
\end{table}

\begin{table}[]
	\caption{Results of the methods, new}
	\label{tab:results}
	\begin{tabular}{l|lllll}
		& Otsu    & Local Otsu & Sauvola & Niblack & \textbf{Proposed} \\ \hline
		F-measure  & 0.07265 & 0.51266    & 0.19074 & 0.15676 & \textbf{0.8670}  \\
		pF-measure & 0.27118 & 0.52280    & 0.24581 & 0.14138 & \textbf{0.8720}  \\
		PSNR       & 1.55566 & 14.78624   & 6.27023 & 4.90463 & \textbf{21.3200} \\
		%NRM        & 0.50156 & 0.24226    & 0.44956 & 0.46181 & \textbf{0.0446}  \\
		%MPM        & 0.44865 & 0.00064    & 0.07627 & 0.19015 & \textbf{0.0001}  \\
		DRD        & 0.00010 & 0.01080    & 0.00001 & 0.00001 & \textbf{0.0240} 
	\end{tabular}
\end{table}


\begin{figure}[h]
	\centering
	\begin{subfigure}{.23\textwidth}
		\fbox{\includegraphics[width=.99\linewidth]{images/boxplot/F-measure.png} }
		\subcaption{F-measure}
	\end{subfigure}
	\begin{subfigure}{.23\textwidth}
		\fbox{\includegraphics[width=.99\linewidth]{images/boxplot/pF-measure.png} }
		\subcaption{pF-measure}
	\end{subfigure}
	\begin{subfigure}{.23\textwidth}
		\fbox{\includegraphics[width=.99\linewidth]{images/boxplot/PSNR.png} }
		\subcaption{PSNR}	
	\end{subfigure}
	\begin{subfigure}{.23\textwidth}	
		\fbox{\includegraphics[width=.99\linewidth]{images/boxplot/DRD.png} }
		\subcaption{DRD}
	\end{subfigure}
	\begin{subfigure}{.23\textwidth}	
		\fbox{\includegraphics[width=.99\linewidth]{images/boxplot/MPM.png} }
		\subcaption{MPM}
	\end{subfigure}
	\begin{subfigure}{.23\textwidth}	
		\fbox{\includegraphics[width=.99\linewidth]{images/boxplot/NRM.png} }
		\subcaption{NRM}
	\end{subfigure}
	\caption{Result plots}
	\label{fig:boxplot}
\end{figure}
